Multi-Modal Domain Adaptation Across Video Scenes for Temporal Video Grounding

Temporal Video Grounding (TVG) aims to localize the temporal boundary of a specific segment in an untrimmed video based on a given language query. Since datasets in this domain are often gathered from limited video scenes, models tend to overfit to scene-specific factors, which leads to suboptimal performance when encountering new scenes in real-world applications. In a new scene, the fine-grained annotations are often insufficient due to the expensive labor cost, while the coarse-grained video-query pairs are easier to obtain. Thus, to address this issue and enhance model performance on new scenes, we explore the TVG task in an unsupervised domain adaptation (UDA) setting across scenes for the first time, where the video-query pairs in the source scene (domain) are labeled with temporal boundaries, while those in the target scene are not. Under the UDA setting, we introduce a novel Adversarial Multi-modal Domain Adaptation (AMDA) method to adaptively adjust the model's scene-related knowledge by incorporating insights from the target data. Specifically, we tackle the domain gap by utilizing domain discriminators, which help identify valuable scene-related features effective across both domains. Concurrently, we mitigate the semantic gap between different modalities by aligning video-query pairs with related semantics. Furthermore, we employ a mask-reconstruction approach to enhance the understanding of temporal semantics within a scene. Extensive experiments on Charades-STA, ActivityNet Captions, and YouCook2 demonstrate the effectiveness of our proposed method.

==> experiment/qualitative.tex <==

% \begin{figure}[tb]
% \includegraphics[width=\linewidth]{figures/qualitative.pdf}
%     \caption{Qualitative examples on the ActivityNet Captions (sport->household) and the Charades-STA (kitchen->bedroom).}
%     \label{fig:qualitative}
% \end{figure}

% \subsection{Qualitative Analysis}
% The qualitative evaluation results are depicted in the appendix.
% In order to qualitatively evaluate the performance of the AMDA method, we show the qualitative examples on the two datasets in Figure~\ref{fig:qualitative}. In these two cases, the source-only method fails to localize accurate boundaries since it cannot learn \textit{household}-related and \textit{bedroom}-related contexts of the target domains. In comparison, the AMDA model can make more accurate predictions with the guidance of unlabeled target data. Moreover, these two examples show that the AMDA model can predict long-range and short-range segments well.

\subsection{Qualitative Analysis}
The qualitative evaluation results are depicted in the appendix.
% \paragraph{\textbf{Qualitative Comparison}} 
% To assess the AMDA method's performance qualitatively, we provide examples from the three datasets in Figure \ref{fig:qualitative}. In these instances, the source-only method fails to accurately localize boundaries due to its inability to learn from the target domains. In contrast, the AMDA model can make more precise predictions with the aid of unlabeled target data. Furthermore, these examples demonstrate that the AMDA model can predict both long-range and short-range segments effectively.

% \paragraph{\textbf{Failure Cases}}
% Despite its outstanding performance compared to other UDA methods, AMDA may still fail in certain cases, as illustrated in Figure~\ref{fig:failure_case}. (a) In this instance, the query is asking for the second occurrence of action "weld the item," while AMDA returns the answer segment for the first occurrence of welding. This indicates that our model has yet to fully explore temporal semantics. (b) In this case, an out-of-domain subject (an animal) appears in the query, which hinders the prediction. (c) In this instance, the target segment is too short to be accurately detected, and the model appears to generate predictions randomly.
